SIXO: Smoothing Inference with Twisted Objectives

Sequential Monte Carlo (SMC) is an inference algorithm for state space models that approximates the posterior by sampling from a sequence of target distributions. The target distributions are often chosen to be the filtering distributions, but these ignore information from future observations, leading to practical and theoretical limitations in inference and model learning. We introduce SIXO, a method that instead learns targets that approximate the smoothing distributions, incorporating information from all observations. The key idea is to use density ratio estimation to fit functions that warp the filtering distributions into the smoothing distributions. We then use SMC with these learned targets to define a variational objective for model and proposal learning. SIXO yields provably tighter log marginal lower bounds and offers significantly more accurate posterior inferences and parameter estimates in a variety of domains.

==> alg_tex/smc.tex <==


 \begin{algorithm}[H]
    \label{app:algo:smc}
    \caption{Sequential Monte Carlo}
    \begin{spacing}{1.25}
    \begin{algorithmic}[1]
        \Procedure{SMC}{$\{\gamma_t(\bx_{1:t})\}_{t=1}^{T}$, $\{q_t(\bx_t \mid \bx_{1:t-1})\}_{t=1}^T$, $K$}
        \State $w_0^{1:K} = 1,\hspace{2mm} \widehat{Z}_0=1$
        \For {$t = 1,\ldots, T$}
            \For {$k = 1, \ldots, K$}
                \State $\bx_t^k \sim q_t(\bx_t | \bx_{1:t-1}^k)$
                \State $\bx_{1:t}^k = (\bx_{1:t-1}^k, \bx_t^k)$
                \State $\alpha_t^k = \dfrac{\gamma_t(\bx_{1:t}^k)}{\gamma_t(\bx_{1:t-1}^k)q_t(\bx_t^k \mid \bx_{1:t-1}^k)}$
                \State $w_t^k = w_{t-1}^k\alpha_t^k$
            \EndFor
            \State $\widehat{Z_t/Z_{t-1}} = \dfrac{\sum_{k=1}^K w_{t}^k}{\sum_{k=1}^K w_{t-1}^k}$
            \State $\widehat{Z}_t = \widehat{Z}_{t-1}(\widehat{Z_{t}/Z_{t-1}})$
            \If{should resample}
                \For{$k = 1, \ldots, K$}
                    \State $a_t^k \sim \text{Categorial}(w_t^{1:K})$
                    \State $\tilde{\bx}_{1:t}^k = \bx_{1:t}^{a_t^k}$
                \EndFor
                \State $\bx_{1:t}^{1:K} = \tilde{\bx}_{1:t}^{1:K}$
                \State $w_t^{1:K} = 1$
            \EndIf
        \EndFor
        \State\Return $\widehat{Z}_{1:T}$, $\bx_{1:T}^{1:K}$
        \EndProcedure
    \end{algorithmic}
    \end{spacing}
\end{algorithm}






% \begin{algorithm}[t]
% \caption{Twisted SMC sweep (\textcolor{OliveGreen}{green} terms can be omitted to recover untwisted SMC.)}\label{app:alg:sixo}
% \begin{algorithmic}[1]
% \Require Filtering targets $p_{\btheta}(\bx_{1:t},\by_{1:t})$, proposals $q_{\bphi}(\bx_t \mid \bx_{t-1}, \by_{1:T})$, \textcolor{OliveGreen}{twists $r_{\bpsi}(\bx_t ; \by_{t+1:T})$}, number of particles $N$. 
% \State $\forall i \in (1, \ldots, N)$ define: \quad $w_0^{i} \triangleq 1 / N$, \quad $\bx_0^{i} \triangleq \mathbf{0}$, \quad \textcolor{OliveGreen}{$r_0^{i} \triangleq 1.0$}.
% \For{$t=1 \ldots T$}
% \State Sample ancestors $a_{t-1}^i$ and update $w_{t-1}^i$ using \eqref{equ:smc:ancestor}.
% \State Propose $\bx_{1:t}^{i}$ given $\bx_{1:t-1}^{a_{t-1}^i}$ using $q_{\bphi, t}$ and \eqref{equ:smc:propagation}.
% \State \textcolor{OliveGreen}{\textbf{If} $t < T$ \textbf{then} $r_t^{i} = r_{\bpsi , t} (\bx_t^{i} ; \by_{t+1:T} )$ \textbf{else} $r_t^{i} = 1.0$ } 
% \State Set $w_t^{i} = w_{t-1}^{a_{t-1}^i} \times \alpha_{t}^i$, where $\alpha_t^i$ is defined in \eqref{equ:smc:weight} for SMC and \textcolor{OliveGreen}{\eqref{equ:sixo:weight} for twisted SMC}. % p_{\btheta} \left( \bx_t^{i} , \by_t \mid \bx_{t-1}^{a_{t-1}^{(i)}} \right) \, \textcolor{blue}{r_t^{i}} \, / \, q_{\bphi} \left( \bx_t^{i} \mid \bx_{t-1}^{a_{t-1}^{i}} \right) \textcolor{blue}{r_{t-1}^{a_{t-1}^{i}}} $
% \EndFor
% \State \textbf{return} \, $\lbrace \bx_t^{1:N} \rbrace_{t=1}^T$, \, $\prod_{t=1}^T (1 / N) \sum_{i=1}^N \alpha_t^{i}$  % Not sure why \Return didnt work...
% \end{algorithmic}
% \end{algorithm}




% \begin{algorithm}[t]
% \caption{SIXO SMC Forward Pass}\label{alg:sixo}
% \begin{algorithmic}[1]
% \Require Filtering targets $p_{\btheta}(\bx_{1:t},\by_{1:t})$, proposals $q_{\bphi}(\bx_t \mid \bx_{t-1}, \by_{1:T})$, \textcolor{blue}{twists $r_{\bpsi}(\bx_t \mid \by_{t+1:T})$}, number of particles $N$. 
% \vspace{1em}
% \Statex \algcmtns{Initialization of particles.}
% \For{$i=1 \ldots N$}
% \State Simulate $\bx_1^{(i)}$ from $q_{\bphi}(\bx_1)$
% \State \textcolor{blue}{Set $r_1^{(i)} = r_{\bpsi} \left(\bx_1^{(i)} \mid \by_{2:T} \right)$} \algcmt{Calculate twist (no previous twist at $t=1$).}
% \State Set $w_1^{(i)} = p_{\btheta}\left(\bx_1^{(i)}, \by_1\right)  \textcolor{blue}{\tilde{r}_1^{(i)}} \, / \, q_{\bphi} \left( \bx_1^{(i)} \right)$ \algcmt{Reweight particles.}
% \EndFor
% \vspace{1em}

% \Statex \algcmtns{Iteration over time series.}
% \For{$t=2 \ldots T$}
% \For{$i=1 \ldots N$}
% \State Sample $a_{t-1}^{(i)}$ with $\prb \left( a_{t-1}^{(i)}=j \right) = w_{t-1}^{(j)} \, / \, \sum_\ell w_{t-1}^{(\ell)}$  \algcmt{Resample.}
% \State Sample $\bx_t^{(i)}$ from $q \left(\bx_t \mid \bx_{t-1}^{\left(a_{t-1}^{(i)}\right)} \right)$ \algcmt{Propose extensions.}
% \State Set $\bx_{1:t}^{(i)} = \left( \bx_{1:t-1}^{\left(a_{t-1}^{(i)}\right)}, \bx_t^{(i)} \right)$ \algcmt{Append extension.}
% \vspace{1em}

% \If{\textcolor{blue}{t < T}}
%     \State \textcolor{blue}{Set $r_t^{(i)} = r_{\bpsi} \left(\bx_t^{(i)} \mid \by_{t+1:T} \right)$} \algcmt{Calculate twist.}
% \Else
%     \State \textcolor{blue}{Set $r_t^{(i)} = 1.0$} \algcmt{No final twist.}
% \EndIf
% \State Set $w_t^{(i)} = p_{\btheta} \left( \bx_t^{(i)} , \by_t \mid \bx_{t-1}^{\left(a_{t-1}^{(i)}\right)} \right) \, \textcolor{blue}{r_t^{(i)}} \, / \, q_{\bpsi} \left( \bx_t^{(i)} \mid \bx_{t-1}^{\left(a_{t-1}^{(i)}\right)} \right) \textcolor{blue}{r_{t-1}^{\left(a_{t-1}^{(i)}\right)}} $ \algcmtns{Reweight.}
% \EndFor
% \EndFor
% \vspace{1em}
% \State \textbf{return} \,\, $\prod_{t=1}^T (1 / N) \sum_{i=1}^N w_t^{(i)}$  \algcmt{Return model evidence.} % Not sure why \Return didnt work...
% \end{algorithmic}
% \end{algorithm}
